SafeGen: Mitigating Sexually Explicit Content Generation in Text-to-Image Models

Text-to-image (T2I) models, such as Stable Diffusion, have exhibited remarkable performance in generating high-quality images from text descriptions in recent years. However, text-to-image models may be tricked into generating not-safe-for-work (NSFW) content, particularly in sexually explicit scenarios. Existing countermeasures mostly focus on filtering inappropriate inputs and outputs, or suppressing improper text embeddings, which can block sexually explicit content (e.g., naked) but may still be vulnerable to adversarial prompts -- inputs that appear innocent but are ill-intended. In this paper, we present SafeGen, a framework to mitigate sexual content generation by text-to-image models in a text-agnostic manner. The key idea is to eliminate explicit visual representations from the model regardless of the text input. In this way, the text-to-image model is resistant to adversarial prompts since such unsafe visual representations are obstructed from within. Extensive experiments conducted on four datasets and large-scale user studies demonstrate SafeGen's effectiveness in mitigating sexually explicit content generation while preserving the high-fidelity of benign images. SafeGen outperforms eight state-of-the-art baseline methods and achieves 99.4% sexual content removal performance. Furthermore, our constructed benchmark of adversarial prompts provides a basis for future development and evaluation of anti-NSFW-generation methods.

==> sections/relatedwork.tex <==
\section{Related Work}
% 除了传统意义上的unsafe，有一些基于优化的构造攻击
% 被对抗样本攻击
% 后门攻击
\subsection{Attacks on Text-to-Image (T2I) Models}
The susceptibility of T2I models to generating NSFW content, particularly explicit nudity, has been a significant concern~\cite{AI_porn,brack2023mitigating,bird2023typology}. This issue has spurred investigations into various attack vectors targeting these models, such as red-teaming the SD model for unsafe image generation~\cite{rando2022red} through reverse engineering its safety filter mechanism. Moreover, adversarial prompts~\cite{tsai2023ring,yang2023sneakyprompt,gao2023evaluating} were crafted to manipulate T2I models into producing unsafe images, while circumventing detection mechanisms. For instance, Ring-A-Bell~\cite{tsai2023ring} tailors adversarial textual inputs that are conceptually close to the target yet contain nonsense words. Gao \textit{et al.}~\cite{gao2023evaluating} introduced a word-level similarity constraint to mimic realistic human errors, \textit{e.g.}, typo, glyph, and phonetic mistakes. SneakyPrompt~\cite{yang2023sneakyprompt} employs a reinforcement learning-based search approach to craft adversarial prompts, which is effective in maintaining NSFW semantics and alluring SD models to generate unsafe images. Another vulnerability of T2I models is their reliance on large datasets, which are prone to poisoning attacks. Adversaries may release poisoned text-image data on the Internet~\cite{wu2023proactive}, which are then inadvertently collected by data trainers, leading to potential unethical outputs from T2I models.

% \vspace{-5pt}
\subsection{Securing Text-to-Image (T2I) Models}
The generation of pornographic content has highlighted the critical need to regulate T2I models. Current strategies focus on filtering out inappropriate textual inputs or visual outputs and mitigating textually pornographic concepts.

External mitigation measures employ plug-in safety filters~\cite{text_safety_classifier,huggingface_safety_checker} without modifying the T2I model. The main technique is to detect unsafe content during inference or to filter out NSFW data for retraining~\cite{SD-2-1}. Such filters~\cite{text_safety_classifier,huggingface_safety_checker} protect users from exposure to inappropriate content. Similarly, SD-V2.1~\cite{SD-2-1} undergoes complete retraining on censored data using these filters. Nonetheless, existing external approaches suffer from under-generalization and susceptibility to adversarial examples.
Internal mitigation methods alter the T2I model to restrain pornographic textual cues that guide image generation. Existing internal methods are mostly text-dependent. 
The guidance-based SLD~\cite{schramowski2023safe} defines prohibited concepts and steers the classifier-free guidance away from unsafe regions with a new conditioned item.
ESD~\cite{gandikota2023erasing,kim2023towards} fine-tunes the model, where terms like ``nudity'' and ``sexy'' are replaced with ``[blank].''
Unfortunately, these methods have difficulty nullifying connotations in the text input, \textit{e.g.}, the names of porn stars, which are challenging to enumerate and erase.


\textbf{Our Approach.} Unlike prior countermeasures, \sys makes the first attempt to remove representations of visually sexual content from Stable Diffusion in a text-agnostic manner. This effectively cuts off the link between sexually connoted text and visually explicit content. In addition, \sys retains the capability for benign image generation and can seamlessly integrate with existing defense techniques. The efficacy of our design is substantiated through extensive experiments.


==> tables/1_overall.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t!]\centering
\scriptsize
\renewcommand{\arraystretch}{1.2} 
% \resizebox{0.85\linewidth}{!}{
% \begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\tabcolsep}{11pt}
% \setlength{\abovecaptionskip}{0pt}% 
% \setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{\textcolor{red}{Overall performance of \sys against adversarial prompts and comparison with baselines.}}
\begin{tabular}{c|cccccccccc}
\toprule[1.2pt]
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Method}}} & \multicolumn{9}{c}{\textbf{CLIP Score}~$\downarrow$}                                                               \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\textbf{Sneaky}} &
  \multicolumn{1}{c|}{\textbf{Sneaky}} &
  \multicolumn{1}{c|}{\textbf{I2P}} &
  \multicolumn{6}{c}{\textbf{NSFW-56K (With different \# of tokens per prompt )}} \\ \cmidrule{5-10} 
  & \multicolumn{1}{c|}{Prompt-N} & \multicolumn{1}{c|}{Prompt-P} &\multicolumn{1}{c|}{Sexual} &\multicolumn{1}{c}{\textbf{1$\sim$30}} &
  \multicolumn{1}{c}{\textbf{31$\sim$40}} &
  \multicolumn{1}{c}{\textbf{41$\sim$50}} &
  \multicolumn{1}{c}{\textbf{51$\sim$60}} &
  \multicolumn{1}{c}{\textbf{61$\sim$70}} &
  \multicolumn{1}{c}{\textbf{$>$~70}} \\ \midrule[1pt]
Original SD                                                         & \multicolumn{1}{c|}{21.77} & \multicolumn{1}{c|}{20.65} & \multicolumn{1}{c|}{22.39} &   \multicolumn{1}{c}{26.40} &
  \multicolumn{1}{c}{26.56} &
  \multicolumn{1}{c}{27.07} &
  \multicolumn{1}{c}{26.63} &
  \multicolumn{1}{c}{27.56} &
  \multicolumn{1}{c}{25.43} \\ \midrule
SD-V2.1                                                             & \multicolumn{1}{c|}{20.30} & \multicolumn{1}{c|}{19.19} & \multicolumn{1}{c|}{21.75} &   \multicolumn{1}{c}{24.60} &
  \multicolumn{1}{c}{23.66} &
  \multicolumn{1}{c}{24.02} &
  \multicolumn{1}{c}{24.08} &
  \multicolumn{1}{c}{24.81} &
  \multicolumn{1}{c}{22.21} \\ \midrule
Safety Filter                                                       & \multicolumn{1}{c|}{19.01} & \multicolumn{1}{c|}{18.51} & \multicolumn{1}{c|}{19.64} &   \multicolumn{1}{c}{19.99} & 
  \multicolumn{1}{c}{20.07} & 
  \multicolumn{1}{c}{20.33} & 
  \multicolumn{1}{c}{20.89} & 
  \multicolumn{1}{c}{21.43} & 
  \multicolumn{1}{c}{20.65} \\ \midrule
ESD                                                                 & \multicolumn{1}{c|}{19.89} & \multicolumn{1}{c|}{18.12} & \multicolumn{1}{c|}{21.16} &  \multicolumn{1}{c}{24.04} &
  \multicolumn{1}{c}{24.11} &
  \multicolumn{1}{c}{24.59} &
  \multicolumn{1}{c}{24.72} &
  \multicolumn{1}{c}{25.94} &
  \multicolumn{1}{c}{23.79} \\ \midrule
SLD (MAX)                                                           & \multicolumn{1}{c|}{18.63} & \multicolumn{1}{c|}{17.40} & \multicolumn{1}{c|}{19.05} &   \multicolumn{1}{c}{22.74} &
  \multicolumn{1}{c}{22.41} &
  \multicolumn{1}{c}{22.94} &
  \multicolumn{1}{c}{22.75} &
  \multicolumn{1}{c}{23.85} &
  \multicolumn{1}{c}{21.56} \\ \midrule
SLD (STRONG)                                                        & \multicolumn{1}{c|}{19.88} & \multicolumn{1}{c|}{18.45} & \multicolumn{1}{c|}{20.31} &   \multicolumn{1}{c}{23.91} &
  \multicolumn{1}{c}{23.84} &
  \multicolumn{1}{c}{24.49} &
  \multicolumn{1}{c}{24.30} &
  \multicolumn{1}{c}{25.25} &
  \multicolumn{1}{c}{22.92} \\ \midrule
SLD (MEDIUM)                                                        & \multicolumn{1}{c|}{20.89} & \multicolumn{1}{c|}{19.49} & \multicolumn{1}{c|}{21.68} &   \multicolumn{1}{c}{25.30} &
  \multicolumn{1}{c}{25.20} &
  \multicolumn{1}{c}{25.93} &
  \multicolumn{1}{c}{25.40} &
  \multicolumn{1}{c}{26.55} &
  \multicolumn{1}{c}{24.18} \\ \midrule
SLD (WEAK)                                                          & \multicolumn{1}{c|}{21.73} & \multicolumn{1}{c|}{20.50} & \multicolumn{1}{c|}{22.37} &   \multicolumn{1}{c}{26.51} &
  \multicolumn{1}{c}{26.39} &
  \multicolumn{1}{c}{26.83} &
  \multicolumn{1}{c}{26.49} &
  \multicolumn{1}{c}{27.38} &
  \multicolumn{1}{c}{25.10} \\ \midrule
\textbf{\sys(Ours) }                                                 & \multicolumn{1}{c|}{\textbf{16.83}} & \multicolumn{1}{c|}{\textbf{15.46}} & \multicolumn{1}{c|}{\textbf{18.13}} &   \multicolumn{1}{c}{\textbf{16.11}} &
  \multicolumn{1}{c}{\textbf{16.00}} &
  \multicolumn{1}{c}{\textbf{17.37}} &
  \multicolumn{1}{c}{\textbf{17.92}} &
  \multicolumn{1}{c}{\textbf{18.34}} &
  \multicolumn{1}{c}{\textbf{17.19}} \\ \bottomrule[1.2pt]
\end{tabular}
\label{tab:test_overall_sexual}
% \end{threeparttable}}
\end{table*}

==> tables/1_overall_sexual.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}\centering
\resizebox{.95\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\renewcommand{\arraystretch}{1}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{\textcolor{red}{Overall performance of \sys against adversarial prompts and comparison with baselines.}}
\setlength{\tabcolsep}{3mm}{
\begin{tabular}{@{}l|rrrr@{}}
\toprule[1.2pt]
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{CLIP Score}~$\downarrow$}                                                               \\ \cmidrule(l){2-5} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Sneaky}\\ \textbf{Prompt-N}\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Sneaky}\\ \textbf{Prompt-P}\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{I2P}\\ \textbf{(Sexual)}\end{tabular}} &
  \multicolumn{1}{c}{\textbf{NSFW-56k}} \\ \midrule[1pt]
Original SD                                                         & \multicolumn{1}{c|}{21.77} & \multicolumn{1}{c|}{20.65} & \multicolumn{1}{c|}{22.39} & \multicolumn{1}{c}{26.61} \\ \midrule
SD-V2.1                                                             & \multicolumn{1}{c|}{20.30} & \multicolumn{1}{c|}{19.19} & \multicolumn{1}{c|}{21.75} & \multicolumn{1}{c}{23.90}  \\ \midrule
Safety Filter                                                       & \multicolumn{1}{c|}{19.01} & \multicolumn{1}{c|}{18.51} & \multicolumn{1}{c|}{19.64} & \multicolumn{1}{c}{20.56} \\ \midrule
ESD                                                                 & \multicolumn{1}{c|}{19.89} & \multicolumn{1}{c|}{18.12} & \multicolumn{1}{c|}{21.16} & \multicolumn{1}{c}{24.59} \\ \midrule
SLD (MAX)                                                           & \multicolumn{1}{c|}{18.63} & \multicolumn{1}{c|}{17.40} & \multicolumn{1}{c|}{19.05} & \multicolumn{1}{c}{22.71} \\ \midrule
SLD (STRONG)                                                        & \multicolumn{1}{c|}{19.88} & \multicolumn{1}{c|}{18.45} & \multicolumn{1}{c|}{20.31} & \multicolumn{1}{c}{24.12} \\ \midrule
SLD (MEDIUM)                                                        & \multicolumn{1}{c|}{20.89} & \multicolumn{1}{c|}{19.49} & \multicolumn{1}{c|}{21.68} & \multicolumn{1}{c}{25.43} \\ \midrule
SLD (WEAK)                                                          & \multicolumn{1}{c|}{21.73} & \multicolumn{1}{c|}{20.50} & \multicolumn{1}{c|}{22.37} & \multicolumn{1}{c}{26.45} \\ \midrule
\textbf{\sys(Ours) }                                                      & \multicolumn{1}{c|}{\textbf{16.83}} & \multicolumn{1}{c|}{\textbf{15.46}} & \multicolumn{1}{c|}{\textbf{18.13}} & \multicolumn{1}{c}{\textbf{17.16}} \\ 
\bottomrule[1.2pt]
\end{tabular}
}
\label{tab:test_overall_sexual}
\end{threeparttable}}
\end{table}

==> tables/1_overall_sexual_2columns.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}\centering
\resizebox{.85\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\renewcommand{\arraystretch}{0.7}
% \newcolumntype{"}{@{\hskip\tabcolsep\vrule width 0.1pt\hskip\tabcolsep}} 
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
\setlength\tabcolsep{1.5pt}

\caption{\textcolor{red}{Overall performance of \sys against adversarial prompts and comparison with baselines.}}

\setlength{\tabcolsep}{3mm}{
\begin{tabular}{@{}l|cccc|cccc@{}}
\toprule[1.2pt]
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} &
  \multicolumn{4}{c|}{\textbf{CLIP Score $\downarrow$}} &
  \multicolumn{4}{c}{\textbf{Remove Rate $\uparrow$}} \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Sneaky\\ Prompt-N\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Sneaky\\ Prompt-P\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}I2P\\ (Sexual)\end{tabular}}} &
  \textbf{NSFW-56k} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Sneaky\\ Prompt-N\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Sneaky\\ Prompt-P\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}I2P\\ (Sexual)\end{tabular}}} &
  \multicolumn{1}{c}{\textbf{NSFW-56k}} \\ \midrule[1pt]
Original SD &
  \multicolumn{1}{c|}{21.77} &
  \multicolumn{1}{c|}{20.65} &
  \multicolumn{1}{c|}{22.39} &
  26.61 &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c}{-} \\ \midrule
SD-V2.1 &
  \multicolumn{1}{c|}{20.30} &
  \multicolumn{1}{c|}{19.19} &
  \multicolumn{1}{c|}{21.75} &
  23.90 &
  \multicolumn{1}{c|}{58.8\%} &
  \multicolumn{1}{c|}{45.9\%} &
  \multicolumn{1}{c|}{43.8\%} &
  \multicolumn{1}{c}{57.0\%} \\ \midrule
Safety Filter &
  \multicolumn{1}{c|}{19.01} &
  \multicolumn{1}{c|}{18.51} &
  \multicolumn{1}{c|}{19.64} &
  20.56 &
  \multicolumn{1}{c|}{67.9\%} &
  \multicolumn{1}{c|}{67.1\%} &
  \multicolumn{1}{c|}{70.8\%} &
  \multicolumn{1}{c}{70.0\%} \\ \midrule
ESD &
  \multicolumn{1}{c|}{19.89} &
  \multicolumn{1}{c|}{18.12} &
  \multicolumn{1}{c|}{21.16} &
  24.59 &
  \multicolumn{1}{c|}{80.3\%} &
  \multicolumn{1}{c|}{80.6\%} &
  \multicolumn{1}{c|}{59.7\%} &
  \multicolumn{1}{c}{67.6\%} \\ \midrule
SLD (Max) &
  \multicolumn{1}{c|}{18.63} &
  \multicolumn{1}{c|}{17.40} &
  \multicolumn{1}{c|}{19.05} &
  22.71 &
  \multicolumn{1}{c|}{72.7\%} &
  \multicolumn{1}{c|}{69.3\%} &
  \multicolumn{1}{c|}{75.2\%} &
  \multicolumn{1}{c}{60.7\%} \\ \midrule
SLD (Strong) &
  \multicolumn{1}{c|}{19.88} &
  \multicolumn{1}{c|}{18.45} &
  \multicolumn{1}{c|}{20.31} &
  24.12 &
  \multicolumn{1}{c|}{53.3\%} &
  \multicolumn{1}{c|}{44.2\%} &
  \multicolumn{1}{c|}{63.6\%} &
  \multicolumn{1}{c}{41.5\%} \\ \midrule
SLD (Medium) &
  \multicolumn{1}{c|}{20.89} &
  \multicolumn{1}{c|}{19.49} &
  \multicolumn{1}{c|}{21.68} &
  25.43 &
  \multicolumn{1}{c|}{27.6\%} &
  \multicolumn{1}{c|}{22.2\%} &
  \multicolumn{1}{c|}{39.4\%} &
  \multicolumn{1}{c}{20.6\%} \\ \midrule
SLD (Weak) &
  \multicolumn{1}{c|}{21.73} &
  \multicolumn{1}{c|}{20.50} &
  \multicolumn{1}{c|}{22.37} &
  26.45 &
  \multicolumn{1}{c|}{10.9\%} &
  \multicolumn{1}{c|}{7.5\%} &
  \multicolumn{1}{c|}{9.8\%} &
  \multicolumn{1}{c}{5.6\%} \\ \midrule
\textbf{SafeGen (Ours)} &
  \multicolumn{1}{c|}{\textbf{16.83}} &
  \multicolumn{1}{c|}{\textbf{15.46}} &
  \multicolumn{1}{c|}{\textbf{18.13}} &
  \textbf{17.16} &
  \multicolumn{1}{c|}{\textbf{97.8\%}} &
  \multicolumn{1}{c|}{\textbf{97.6\%}} &
  \multicolumn{1}{c|}{\textbf{91.6\%}} &
  \multicolumn{1}{c}{\textbf{99.1\%}} \\ \bottomrule[1.2pt]
\end{tabular}
}

\label{tab:test_overall_sexual}
\end{threeparttable}}
\end{table*}

==> tables/4_hyperparam_lambda.tex <==
% \begin{table}\centering
% \scriptsize
% % \resizebox{.95\linewidth}{!}{
% \begin{threeparttable}[t]
% % \renewcommand{\TPTminimum}{\linewidth}
% \renewcommand{\arraystretch}{1}
% \setlength{\abovecaptionskip}{0pt}% 
% \setlength{\belowcaptionskip}{0pt}%
% \caption{[RQ4-1] Performance of \sys across different hyperparameters $\lambda_1$ and $\lambda_2$ when solely governing the vision-only self-attention layers.}
% % \caption{Ablating different  Performance of \sys When Confronted with Benign COCO-25k Prompts and Comparison with Baselines}
% \setlength{\tabcolsep}{1pt}{
% \begin{tabular}{@{}l|cc|cc@{}}
% \toprule[1.2pt]
% \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} &
%   \multicolumn{1}{c|}{\textbf{NRR (\%) $\uparrow$}} &
%   \textbf{CLIP Score $\downarrow$} &
%   \multicolumn{1}{c|}{\textbf{LPIPS Score $\downarrow$}} &
%   \textbf{CLIP Score $\uparrow$} \\ \cmidrule(l){2-5} 
% \multicolumn{1}{c|}{} &
%   \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Adversarial Prompts\\ (SneakyPrompt-N)\end{tabular}}} &
%   \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Benign Prompts\\ (COCO-25k)\end{tabular}}} \\ \midrule[1pt]
% $\lambda_1:0.1, \lambda_2:0.9$ & \multicolumn{1}{c|}{91.7\%} & 17.79 & \multicolumn{1}{c|}{0.805} & \multicolumn{1}{c}{24.33} \\ \midrule
% $\lambda_1:0.2, \lambda_2:0.8$ & \multicolumn{1}{c|}{93.2\%} & 17.65 & \multicolumn{1}{c|}{0.820} & \multicolumn{1}{c}{23.88} \\ \midrule
% $\lambda_1:0.3, \lambda_2:0.7$ & \multicolumn{1}{c|}{93.5\%} & 17.27 & \multicolumn{1}{c|}{0.845} & \multicolumn{1}{c}{23.79} \\ \midrule
% $\lambda_1:0.4, \lambda_2:0.6$ & \multicolumn{1}{c|}{89.2\%} & 17.93 & \multicolumn{1}{c|}{0.861} & \multicolumn{1}{c}{23.70} \\ \midrule
% $\lambda_1:0.5, \lambda_2:0.5$ & \multicolumn{1}{c|}{93.7\%} & 17.11 & \multicolumn{1}{c|}{0.881} & \multicolumn{1}{c}{23.20} \\ \bottomrule[1.2pt]
% \end{tabular}
% }

% \label{tab:test_hyperparam_lambda}
% \end{threeparttable}
% \end{table}




\begin{table}\centering
\scriptsize
% \resizebox{.95\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\renewcommand{\arraystretch}{1}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{[RQ4] Performance of \sys across different hyperparameters $\lambda_1$ and $\lambda_2$ when solely governing the vision-only self-attention layers.}
% \caption{Ablating different  Performance of \sys When Confronted with Benign COCO-25k Prompts and Comparison with Baselines}

\setlength{\tabcolsep}{3.4mm}{
\begin{tabular}{@{}l|cc|cc@{}}
\toprule[1.2pt]
% \multirow{2}{*}{\textbf{Method}} &
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}} NRR (\%) $\uparrow$\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}CLIP\\ Score $\downarrow$\end{tabular}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}LPIPS\\ Score $\downarrow$\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}CLIP\\ Score $\uparrow$\end{tabular}} \\ \cmidrule(l){2-5} 
 &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Adversarial Prompts\\ (SneakyPrompt-Natural)\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Benign Prompts\\ (COCO-25k)\end{tabular}}} \\ \midrule[1pt]
$\lambda_1:0.1, \lambda_2:0.9$ & \multicolumn{1}{c|}{91.7\%} & 17.79 & \multicolumn{1}{c|}{0.805} & \multicolumn{1}{c}{24.33} \\ \midrule
$\lambda_1:0.2, \lambda_2:0.8$ & \multicolumn{1}{c|}{93.2\%} & 17.65 & \multicolumn{1}{c|}{0.820} & \multicolumn{1}{c}{23.88} \\ \midrule
$\lambda_1:0.3, \lambda_2:0.7$ & \multicolumn{1}{c|}{93.5\%} & 17.27 & \multicolumn{1}{c|}{0.845} & \multicolumn{1}{c}{23.79} \\ \midrule
$\lambda_1:0.4, \lambda_2:0.6$ & \multicolumn{1}{c|}{89.2\%} & 17.93 & \multicolumn{1}{c|}{0.861} & \multicolumn{1}{c}{23.70} \\ \midrule
$\lambda_1:0.5, \lambda_2:0.5$ & \multicolumn{1}{c|}{93.7\%} & 17.11 & \multicolumn{1}{c|}{0.881} & \multicolumn{1}{c}{23.20} \\ \bottomrule[1.2pt]
\end{tabular}
}

\label{tab:test_hyperparam_lambda}
\end{threeparttable}
% }
\end{table}


==> tables/5_hyperparam_scheduler.tex <==
\begin{table}\centering
\scriptsize
\resizebox{1.\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\renewcommand{\arraystretch}{1}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{[RQ4-3] Performance of \sys using different diffusion schedulers during inference.}
% \caption{Ablating different  Performance of \sys When Confronted with Benign COCO-25k Prompts and Comparison with Baselines}

\setlength{\tabcolsep}{3.1mm}{
\begin{tabular}{@{}l|cc|cc@{}}
\toprule[1.2pt]
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Diffusion Scheduler}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}NRR (\%) $\uparrow$\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}CLIP\\ Score $\downarrow$\end{tabular}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}LPIPS\\ Score $\downarrow$\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}CLIP\\ Score $\uparrow$\end{tabular}} \\ \cmidrule(l){2-5} 
\multicolumn{1}{c|}{} &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Adversarial Prompts\\ (SneakyPrompt-Natural)\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Benign Prompts\\ (COCO-25k)\end{tabular}}} \\ \midrule[1pt]
PNDM                   & \multicolumn{1}{c|}{99.0\%} & 19.73 & \multicolumn{1}{c|}{0.7817} & \multicolumn{1}{c}{24.43} \\ \midrule
LMSD                   & \multicolumn{1}{c|}{98.2\%} & 19.82 & \multicolumn{1}{c|}{0.7828} & \multicolumn{1}{c}{24.13} \\ \midrule
EulerDiscrete          & \multicolumn{1}{c|}{99.2\%} & 19.71 & \multicolumn{1}{c|}{0.7850}  & \multicolumn{1}{c}{24.01} \\ \midrule
DPMSovler              & \multicolumn{1}{c|}{99.2\%} & 20.02 & \multicolumn{1}{c|}{0.7770}  & \multicolumn{1}{c}{24.11} \\ \midrule
DDIM                   & \multicolumn{1}{c|}{98.3\%} & 19.89 & \multicolumn{1}{c|}{0.7802} & \multicolumn{1}{c}{24.22} \\ \midrule
DDPM                   & \multicolumn{1}{c|}{98.2\%} & 19.76 & \multicolumn{1}{c|}{0.7941} & \multicolumn{1}{c}{24.21} \\ \midrule
EulerAncestorDiscrete & \multicolumn{1}{c|}{98.2\%} & 19.95 & \multicolumn{1}{c|}{0.7960}  & \multicolumn{1}{c}{24.02} \\ \bottomrule[1.2pt]
\end{tabular}
}


\label{tab:test_hyperparam_scheduler}
\end{threeparttable}
}
\end{table}


==> tables/5_hyperparam_scheduler_SLD.tex <==
\begin{table}\centering
\footnotesize
% \resizebox{0.95\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\renewcommand{\arraystretch}{1}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{[RQ4-3] Performance of \sys using different diffusion schedulers during inference.}
% \caption{Ablating different  Performance of \sys When Confronted with Benign COCO-25k Prompts and Comparison with Baselines}

\setlength{\tabcolsep}{2.8mm}{
\begin{tabular}{@{}l|cc|cc@{}}
\toprule[1.2pt]
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Diffusion Scheduler}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}NRR (\%) $\uparrow$\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}CLIP\\ Score $\downarrow$\end{tabular}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}LPIPS\\ Score $\downarrow$\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}CLIP\\ Score $\uparrow$\end{tabular}} \\ \cmidrule(l){2-5} 
\multicolumn{1}{c|}{} &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Adversarial Prompts\\ (SneakyPrompt-Natural)\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Benign Prompts\\ (COCO-25k)\end{tabular}}} \\ \midrule[1pt]
PNDM                   & \multicolumn{1}{c|}{\tblue{99.1\%}} & 17.85 & \multicolumn{1}{c|}{0.789} & \multicolumn{1}{c}{24.60} \\ \midrule
LMSD                   & \multicolumn{1}{c|}{\tblue{98.0\%}} & 18.31 & \multicolumn{1}{c|}{0.792} & \multicolumn{1}{c}{24.40} \\ \midrule
EulerDiscrete          & \multicolumn{1}{c|}{\tblue{99.3\%}} & 18.52 & \multicolumn{1}{c|}{0.794}  & \multicolumn{1}{c}{24.42} \\ \midrule
EulerAncestorDiscrete              & \multicolumn{1}{c|}{\tblue{98.7\%}} & 17.98 & \multicolumn{1}{c|}{0.811}  & \multicolumn{1}{c}{24.54} \\ \midrule
DPMSovler                  & \multicolumn{1}{c|}{\tblue{99.1\%}} & 18.70 & \multicolumn{1}{c|}{0.786} & \multicolumn{1}{c}{24.44} \\ \midrule
DDPM                   & \multicolumn{1}{c|}{\tblue{98.2\%}} & 17.97 & \multicolumn{1}{c|}{0.810} & \multicolumn{1}{c}{24.40} \\ \midrule
DDIM                   & \multicolumn{1}{c|}{\tblue{98.7\%}} & 18.50 & \multicolumn{1}{c|}{0.789}  & \multicolumn{1}{c}{24.49} \\ \bottomrule[1.2pt]
\end{tabular}
}
\label{tab:test_hyperparam_scheduler}
\vspace{-15pt}
\end{threeparttable}
\end{table}


==> tables/6_hyperparam_steps.tex <==
\begin{table}\centering
\scriptsize
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\renewcommand{\arraystretch}{1}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{[RQ4-2]~Performance of \sys with different denoising diffusion steps during inference.}
% \caption{Ablating different  Performance of \sys When Confronted with Benign COCO-25k Prompts and Comparison with Baselines}
\setlength{\tabcolsep}{4.3mm}{
\begin{tabular}{@{}c|cc|cc@{}}
\toprule[1.2pt]
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Steps \end{tabular}}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}NRR (\%) $\uparrow$\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}CLIP\\ Score $\downarrow$\end{tabular}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}LPIPS\\ Score $\downarrow$\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}CLIP\\ Score $\uparrow$\end{tabular}} \\ \cmidrule(l){2-5} 
\multicolumn{1}{c|}{} &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Adversarial Prompts\\ (SneakyPrompt-Natural)\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Benign Prompts\\ (COCO-25k)\end{tabular}}} \\ \midrule[1pt]
25  & \multicolumn{1}{c|}{99.2\%} & 19.54 & \multicolumn{1}{c|}{0.8187} & 23.68 \\ \midrule
50  & \multicolumn{1}{c|}{98.2\%} & 19.95 & \multicolumn{1}{c|}{0.7962} & 24.02 \\ \midrule
75  & \multicolumn{1}{c|}{98.3\%} & 19.95 & \multicolumn{1}{c|}{0.7900} & 24.43 \\ \midrule
100 & \multicolumn{1}{c|}{98.2\%} & 20.19 & \multicolumn{1}{c|}{0.7863} & 24.28 \\ \midrule
125 & \multicolumn{1}{c|}{98.7\%} & 20.13 & \multicolumn{1}{c|}{0.7862} & 24.08 \\ \midrule
150 & \multicolumn{1}{c|}{99.3\%} & 19.93 & \multicolumn{1}{c|}{0.7856} & 24.16 \\ \bottomrule[1.2pt]
\end{tabular}
}
\label{tab:test_hyperparam_infersteps}
\end{threeparttable}
% }
\end{table}


==> tables/6_hyperparam_steps_SLD.tex <==
\begin{table}\centering
\footnotesize
% \resizebox{0.98\linewidth}{!}{
\begin{threeparttable}[h]
% \renewcommand{\TPTminimum}{\linewidth}
\renewcommand{\arraystretch}{1}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{[RQ4-4]~Performance of \sys with different denoising diffusion steps during inference.}
% \caption{Ablating different  Performance of \sys When Confronted with Benign COCO-25k Prompts and Comparison with Baselines}
\setlength{\tabcolsep}{4.3mm}{
\begin{tabular}{@{}c|cc|cc@{}}
\toprule[1.2pt]
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Steps \end{tabular}}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}NRR (\%) $\uparrow$\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}CLIP\\ Score $\downarrow$\end{tabular}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}LPIPS\\ Score $\downarrow$\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}CLIP\\ Score $\uparrow$\end{tabular}} \\ \cmidrule(l){2-5} 
\multicolumn{1}{c|}{} &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Adversarial Prompts\\ (SneakyPrompt-Natural)\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Benign Prompts\\ (COCO-25k)\end{tabular}}} \\ \midrule[1pt]
25  & \multicolumn{1}{c|}{\tblue{99.5\%}} & 17.12 & \multicolumn{1}{c|}{0.794} & \multicolumn{1}{c}{24.16} \\ \midrule
50  & \multicolumn{1}{c|}{\tblue{99.0\%}} & 17.85 & \multicolumn{1}{c|}{0.789} & \multicolumn{1}{c}{24.58} \\ \midrule
75  & \multicolumn{1}{c|}{\tblue{92.8\%}} & 18.47 & \multicolumn{1}{c|}{0.786} & \multicolumn{1}{c}{24.53} \\ \midrule
100 & \multicolumn{1}{c|}{\tblue{99.0\%}} & 18.73 & \multicolumn{1}{c|}{0.792} & \multicolumn{1}{c}{24.47} \\ \midrule
125 & \multicolumn{1}{c|}{\tblue{92.8\%}} & 18.62 & \multicolumn{1}{c|}{0.792} & \multicolumn{1}{c}{24.46} \\ \midrule
150 & \multicolumn{1}{c|}{\tblue{92.8\%}} & 19.37 & \multicolumn{1}{c|}{0.776} & \multicolumn{1}{c}{24.50} \\ \bottomrule[1.2pt]
\end{tabular}
}
\label{tab:test_hyperparam_infersteps}
\end{threeparttable}
% }
\end{table}


==> tables/7_hyparam_prompt_TokenNums.tex <==
\begin{table}\centering
\resizebox{.95\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\renewcommand{\arraystretch}{1}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
\setlength\tabcolsep{4.5pt}
\caption{\textcolor{red}{The performance of \sys using different diffusion steps for inference}.}
% \caption{Ablating different  Performance of \sys When Confronted with Benign COCO-25k Prompts and Comparison with Baselines}

\setlength{\tabcolsep}{3mm}{
\begin{tabular}{@{}l|cccccc@{}}
\toprule[1.2pt]
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Token \\ Numbers\end{tabular}}}} &
  \multicolumn{6}{c}{\textbf{CLIP Score $\downarrow$ \textcolor{red}{(on NSFW-56k)} }} \\ \cmidrule(l){2-7} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\textbf{1$\sim$30}} &
  \multicolumn{1}{c|}{\textbf{31$\sim$40}} &
  \multicolumn{1}{c|}{\textbf{41$\sim$50}} &
  \multicolumn{1}{c|}{\textbf{51$\sim$60}} &
  \multicolumn{1}{c|}{\textbf{61$\sim$70}} &
  \multicolumn{1}{c}{\textbf{$>$~70}} \\ \midrule[1pt]
Original SD &
  \multicolumn{1}{c|}{26.40} &
  \multicolumn{1}{c|}{26.56} &
  \multicolumn{1}{c|}{27.07} &
  \multicolumn{1}{c|}{26.63} &
  \multicolumn{1}{c|}{27.56} &
  \multicolumn{1}{c}{25.43} \\ \midrule
SD-V2.1 &
  \multicolumn{1}{c|}{24.60} &
  \multicolumn{1}{c|}{23.66} &
  \multicolumn{1}{c|}{24.02} &
  \multicolumn{1}{c|}{24.08} &
  \multicolumn{1}{c|}{24.81} &
  \multicolumn{1}{c}{22.21} \\ \midrule
Safety Filter & 
  \multicolumn{1}{c|}{19.99} & 
  \multicolumn{1}{c|}{20.07} & 
  \multicolumn{1}{c|}{20.33} & 
  \multicolumn{1}{c|}{20.89} & 
  \multicolumn{1}{c|}{21.43} & 
  \multicolumn{1}{c}{20.65} \\ \midrule
ESD &
  \multicolumn{1}{c|}{24.04} &
  \multicolumn{1}{c|}{24.11} &
  \multicolumn{1}{c|}{24.59} &
  \multicolumn{1}{c|}{24.72} &
  \multicolumn{1}{c|}{25.94} &
  \multicolumn{1}{c}{23.79} \\ \midrule
SLD (Max) &
  \multicolumn{1}{c|}{22.74} &
  \multicolumn{1}{c|}{22.41} &
  \multicolumn{1}{c|}{22.94} &
  \multicolumn{1}{c|}{22.75} &
  \multicolumn{1}{c|}{23.85} &
  \multicolumn{1}{c}{21.56} \\ \midrule
SLD (Strong) &
  \multicolumn{1}{c|}{23.91} &
  \multicolumn{1}{c|}{23.84} &
  \multicolumn{1}{c|}{24.49} &
  \multicolumn{1}{c|}{24.30} &
  \multicolumn{1}{c|}{25.25} &
  \multicolumn{1}{c}{22.92} \\ \midrule
SLD (Medium) &
  \multicolumn{1}{c|}{25.30} &
  \multicolumn{1}{c|}{25.20} &
  \multicolumn{1}{c|}{25.93} &
  \multicolumn{1}{c|}{25.40} &
  \multicolumn{1}{c|}{26.55} &
  \multicolumn{1}{c}{24.18} \\ \midrule
SLD (Weak) &
  \multicolumn{1}{c|}{26.51} &
  \multicolumn{1}{c|}{26.39} &
  \multicolumn{1}{c|}{26.83} &
  \multicolumn{1}{c|}{26.49} &
  \multicolumn{1}{c|}{27.38} &
  \multicolumn{1}{c}{25.10} \\ \midrule
\textbf{\sys (Ours)} &
  \multicolumn{1}{c|}{\textbf{16.11}} &
  \multicolumn{1}{c|}{\textbf{16.00}} &
  \multicolumn{1}{c|}{\textbf{17.37}} &
  \multicolumn{1}{c|}{\textbf{17.92}} &
  \multicolumn{1}{c|}{\textbf{18.34}} &
  \multicolumn{1}{c}{\textbf{17.19}} \\ \bottomrule[1.2pt]
\end{tabular}
}

\label{tab:test_hyperparam_tokennums}
\end{threeparttable}}
\end{table}

